Diffusion-based Speech Enhancement with Schr\"odinger Bridge and Symmetric Noise Schedule

Recently, diffusion-based generative models have demonstrated remarkable performance in speech enhancement tasks. However, these methods still encounter challenges, including the lack of structural information and poor performance in low Signal-to-Noise Ratio (SNR) scenarios. To overcome these challenges, we propose the Schr\"oodinger Bridge-based Speech Enhancement (SBSE) method, which learns the diffusion processes directly between the noisy input and the clean distribution, unlike conventional diffusion-based speech enhancement systems that learn data to Gaussian distributions. To enhance performance in extremely noisy conditions, we introduce a two-stage system incorporating ratio mask information into the diffusion-based generative model. Our experimental results show that our proposed SBSE method outperforms all the baseline models and achieves state-of-the-art performance, especially in low SNR conditions. Importantly, only a few inference steps are required to achieve the best result.

==> related_work.tex <==
\section{Related Works}
\subsection{Diffusion-based Speech Enhancement}
Diffusion-based speech enhancement task aims to generate the enhanced speech conditioned on the noisy input, which can be seen as a conditional generative task. \cite{lu2021study} pioneered the application of diffusion generative models to the speech enhancement domain by introducing DiffuSE, which generates enhanced waveform using denoising diffusion probabilistic model (DDPM). The original DDPM can only deal with Gaussian noise, to deal with non-Gaussian and non-stationary noise they further designed a conditional diffusion probabilistic model (CDiffuSE) (\cite{lu2022conditional}), which is a generalized version of diffusion probabilistic model that incorporates real noise into the forward process. Another diffusion-based generative method is the score-based Stochastic differential equation (score SDE). \cite{richter2023speech} proposed a score-based SDE generative model for speech enhancement (SGMSE), in which a drift term is introduced to adapt to the conditional reconstruction task. To deal with different kinds of disturbance in speech audio, \cite{serra2022universal} designed a speech enhancement system that contains a conditioning network to provide necessary speech embedding and a score-based generative model to generate the enhanced speech. They show that this system can tackle 55 different distortions. Furthermore, these diffusion models built upon additive Gaussian noise for the forward and reverse process, \cite{yen2023cold} leverages the cold diffusion that considers a more degradation process than the original diffusion process to recover clean speech corrupted by different degradation.

However, current diffusion-based speech enhancement methods encounter challenges due to the lack of structural information for inference and poor performance under low SNR conditions. Our work addresses these challenges by integrating the Schrodinger Bridge and ratio mask into the diffusion process.


\subsection{Schrödinger bridge}
Schrodinger Bridge problem(\cite{schrodinger1932theorie}, \cite{chen2021likelihood}) is to find the optimal method for transforming one probability distribution into another. Many computational frameworks have been proposed to solve the Shrodinger bridge problem and make the Shrodinger bridge tractable (\cite{chen2021likelihood}, \cite{de2021diffusion}, \cite{shi2024diffusion}). In their research, \cite{liu20232} introduced the Image-to-Image Schrodinger Bridge (I$^2$SB), a novel approach for directly learning the nonlinear diffusion processes between two given distributions. This method leverages a score-based generative model to simulate the forward and reverse process of the Schrodinger Bridge. The I$^2$SB model is notable for producing interpretable results and demonstrating superior performance compared to conventional conditional diffusion models. In the work of \cite{chen2023schrodinger}, they introduce the Schrodinger Bridge into the text-to-speech synthesis task. They build a fully tractable Schrodinger bridge to generate a target mel-spectrogram based on the clean text latent representation. Additionally, this work investigates the optimization of noise schedules and sampling processes, enhancing the model's capability to achieve state-of-the-art quality in speech generation and surpass existing diffusion-based models.

In this paper, we leverage the Schrodinger bridge for speech enhancement tasks, aiming to start the iterative inference process directly from noisy input.
